Dolphin: A Challenging and Diverse Benchmark for Arabic NLG

We present Dolphin, a novel benchmark that addresses the need for a natural language generation (NLG) evaluation framework dedicated to the wide collection of Arabic languages and varieties. The proposed benchmark encompasses a broad range of 13 different NLG tasks, including dialogue generation, question answering, machine translation, summarization, among others. Dolphin comprises a substantial corpus of 40 diverse and representative public datasets across 50 test splits, carefully curated to reflect real-world scenarios and the linguistic richness of Arabic. It sets a new standard for evaluating the performance and generalization capabilities of Arabic and multilingual models, promising to enable researchers to push the boundaries of current methodologies. We provide an extensive analysis of Dolphin, highlighting its diversity and identifying gaps in current Arabic NLG research. We also offer a public leaderboard that is both interactive and modular and evaluate several models on our benchmark, allowing us to set strong baselines against which researchers can compare.

==> Acknow.tex <==
% \section{Analysis and Discussion}\label{sec:disc}

\section*{Acknowledgements}\label{sec:acknow}
% We gratefully acknowledge support from the Natural Sciences and Engineering Research Council of Canada (NSERC; RGPIN-2018-04267), the Social Sciences and Humanities Research Council of Canada (SSHRC; 435-2018-0576; 895-2020-1004; 895-2021-1008), Canadian Foundation for Innovation (CFI; 37771), Compute Canada (CC), and \footnote{\href{https://www.computecanada.ca}{https://www.computecanada.ca}} UBC ARC-Sockeye,\footnote{\href{https://arc.ubc.ca/ubc-arc-sockeye}{https://arc.ubc.ca/ubc-arc-sockeye}}. Any opinions, conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of NSERC, SSHRC, CFI, CC, AMD, or UBC ARC-Sockeye. 

% {Acknowledgements}\label{sec:acknow}
We gratefully acknowledge support from Canada Research Chairs (CRC), the Natural Sciences and Engineering Research Council of Canada (NSERC; RGPIN-2018-04267), the Social Sciences and Humanities Research Council of Canada (SSHRC; 435-2018-0576; 895-2020-1004; 895-2021-1008), Canadian Foundation for Innovation (CFI; 37771), Digital Research Alliance of Canada,\footnote{\href{https://alliancecan.ca}{https://alliancecan.ca}} UBC ARC-Sockeye,\footnote{\href{https://arc.ubc.ca/ubc-arc-sockeye}{https://arc.ubc.ca/ubc-arc-sockeye}} and Google TPU Research Cloud (TRC).\footnote{\href{https://sites.research.google/trc/about/}{https://sites.research.google/trc/about/}} Any opinions, conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of CRC, NSERC, SSHRC, CFI, DRAG, Google, or UBC ARC-Sockeye.

==> dolphinAnalysis.tex <==

\section{\dolphin-Based Analysis of Arabic NLG}\label{sec:dolphinAnalys}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \mam{What do we learn from Dolphin? Any gaps in the literature? Need of some tasks and datasets for these tasks? Need for data representing certain domains/genres, data representing certain varieties of Arabic? We should delve deeper here and this should be one of the major sections of the paper.}

\noindent{\textbf{Task Coverage.}} Despite Dolphin's comprehensive coverage of $13$ diverse NLG tasks in various Arabic varieties, it is important to acknowledge that there are currently no available datasets, regardless of accessibility, for NLG tasks such as slide generation, text simplification, nor reasoning. On the positive side, development of~\dolphin~allows us to clearly identify these gaps as future areas for research.

\noindent{\textbf{Distribution of Varieties.}} To illustrate the linguistic diversity encompassed by~\dolphin, an examination of the datasets within Dolphin reveals that MSA holds the largest representation, accounting for \hl{xx\% of the datasets. Dialectal varieties follow with xx\%, while Arabizi and CA make up xx\% and xx\% respectively}. For further information please refer to Table~\ref{tab:dolphin-stats_vara} in the Appendix~\ref{app:dolphin_var}. 

\noindent{\textbf{Orthographic Variation.}} Absence of standardized rules for written Arabic dialects~\cite{habash2012conventional} has resulted in a range of orthographic traditions, both in the context of Latinized writing~\cite{seddah2020building} (i.e., Arabizi) and Arabic contexts. A focal point for different Arabic datasets across countries and varieties, ~\dolphin~offers opportunities for studying these traditions.
% \moa{When people write dialects, they do not agree and there are no rules. Efforts have been made to standardize dialectal texts (e.g., CODA \newcite{habash2012conventional}). Arabizi is a script-based variation. There may be different norms as to how people from each country write their dialect in Latin script~\cite{seddah2020building}.  We highlight the fact that we did not run any normalizer on the data before modeling. }




==> draft.tex <==

%For this task, we use four publicly available QA datasets: (1) The Arabic QA dataset ARCD~\cite{mozannar2019neural}, and the Arabic section of three human-translated Arabic QA test sets of the XTREME multilingual benchmark~\cite{pmlr-v119-hu20b}: (1) MLQA~\cite{lewis2019mlqa}, (2) XQuAD~\cite{artetxe2020cross}, and  (3) TyDi QA~\cite{artetxe2020cross}. For all other test sets, we fine-tune on the Arabic machine-translated SQuAD (AR-XTREME) from the XTREME and test on the human-translated test sets listed above.


 


%We follow the same splits they used where we fine-tune on Arabic SQuAD (Mozannar et al., 2019) and 50\% of ARCD and test on the remaining 50\% of ARCD (ARCD-test). For all the experiments, we fine-tune on the Arabic machine-translated SQuAD (AR-XTREME) from the XTREME multilingual benchmark~\cite{pmlr-v119-hu20b} and we test on the human the four test sets listed above.


% We follow the same splits they used where we fine-tune on Arabic SQuAD (Mozannar et al., 2019) and 50\% of ARCD and test on the remaining 50\% of ARCD (ARCD-test). For all other experiments, we fine-tune on the Arabic machine-translated SQuAD (AR-XTREME) from the XTREME multilingual benchmark (Hu et al., 2020) and test on the human translated test sets listed above.






